Joint Scheduling and Coding For Low In-Order Delivery Delay Over Lossy Paths With Delayed Feedback

We consider the transmission of packets across a lossy end-to-end network path so as to achieve low in-order delivery delay. This can be formulated as a decision problem, namely deciding whether the next packet to send should be an information packet or a coded packet. Importantly, this decision is made based on delayed feedback from the receiver. While an exact solution to this decision problem is challenging, we exploit ideas from queueing theory to derive scheduling policies based on prediction of a receiver queue length that, while suboptimal, can be efficiently implemented and offer substantially better performance than state of the art approaches. We obtain a number of useful analytic bounds that help characterise design trade-offs and our analysis highlights that the use of prediction plays a key role in achieving good performance in the presence of significant feedback delay. Our approach readily generalises to networks of paths and we illustrate this by application to multipath transport scheduler design.

==> figures/Qt_roQr/bound_mu.tikz.tex <==
\pgfplotstableread{../figures/data/bound_mu_p01.dat}{\datasetuno} 
\pgfplotstableread{../figures/data/bound_mu_p06.dat}{\datasetdos} 
\begin{tikzpicture} 
font = \scriptsize, 
\begin{axis}[scale only axis, 
width=\figurewidth,
height=\figureheight,
mark options={solid},
%ymin=0,
%ymax=80,
xmin=0,
xmax=100,
%xtick={0,10,20,30,40,50},
%xticklabels={100,110,120,130,140,150},
ylabel={$\hat{Q}^r_{\text{max}}$},
xlabel={delay (slots)},
compat=1.3,
%xlabel style={name=xlabel},
%ylabel style={name=ylabel, at={(-0.12, 0.5)}},
legend style={ cells = {anchor=center}, at= {(0.25, 0.5)}, anchor = south, draw=none, fill=none,legend columns=1, font = \footnotesize}
]



%\addplot [color=black, solid,line width=0.8pt]
\addplot [color=black]
plot[]
table[x index = 0, y index =1] from \datasetuno;
\addlegendentry{$p=0.6$} 

\addplot [color=black]
plot[]
table[x index = 0, y index =1] from \datasetdos;
\addlegendentry{$p=0.1$} 

\addplot [color=black, dotted]
plot[]
table[x index = 0, y index =2] from \datasetuno;
\addlegendentry{\emph{Bound }} 


\end{axis}



\end{tikzpicture}

==> figures/data/bound_mu_q09_p06.tex <==
1.0000	1.0000	 1.2  1.896017
2.0000	2.0000	 2.4  2.681372
3.0000	2.0000	  3.6  3.283997
4.0000	2.0000	  4.8  3.792033
5.0000	3.0000	  6.0  4.239622
6.0000	3.0000	  7.2  4.644273
7.0000	3.0000	  8.4  5.016388
8.0000	3.0000	  9.6  5.362745
9.0000	4.0000	10.8  5.688050
10.0000	3.0000	12.0  5.995731
11.0000	3.0000	13.2  6.288375
12.0000	3.0000	14.4  6.567994
13.0000	4.0000	15.6  6.836185
14.0000	4.0000	16.8  7.094244
15.0000	4.0000	18.0  7.343240
16.0000	4.0000	19.2  7.584066
17.0000	4.0000	20.4  7.817476
18.0000	5.0000	21.6  8.044117
19.0000	5.0000	22.8  8.264545
20.0000	4.0000	24.0  8.479244
21.0000	4.0000	25.2  8.688639
22.0000	5.0000	26.4  8.893106
23.0000	5.0000	27.6  9.092976
24.0000	5.0000	28.8  9.288546
25.0000	5.0000	30.0  9.480083
26.0000	5.0000	31.2  9.667825
27.0000	5.0000	32.4  9.851991
28.0000	5.0000	33.6 10.032777
29.0000	5.0000	34.8 10.210362
30.0000	5.0000	36.0 10.384910
31.0000	5.0000	37.2 10.556573
32.0000	5.0000	38.4 10.725489
33.0000	5.0000	39.6 10.891786
34.0000	5.0000	40.8 11.055581
35.0000	5.0000	42.0 11.216985
36.0000	6.0000	43.2 11.376099
37.0000	6.0000	44.4 11.533018
38.0000	6.0000	45.6 11.687831
39.0000	6.0000	46.8 11.840620
40.0000	6.0000	48.0 11.991462
41.0000	6.0000	49.2 12.140429
42.0000	6.0000	50.4 12.287592
43.0000	6.0000	51.6 12.433012
44.0000	6.0000	52.8 12.576751
45.0000	6.0000	54.0 12.718866
46.0000	6.0000	55.2 12.859410
47.0000	6.0000	56.4 12.998435
48.0000	7.0000	57.6 13.135988
49.0000	7.0000	58.8 13.272116
50.0000	6.0000	60.0 13.406862
51.0000	6.0000	61.2 13.540266
52.0000	7.0000	62.4 13.672370
53.0000	6.0000	63.6 13.803209
54.0000	7.0000	64.8 13.932819
55.0000	7.0000	66.0 14.061235
56.0000	7.0000	67.2 14.188489
57.0000	7.0000	68.4 14.314611
58.0000	7.0000	69.6 14.439632
59.0000	7.0000	70.8 14.563579
60.0000	6.0000	72.0 14.686481
61.0000	7.0000	73.2 14.808363
62.0000	7.0000	74.4 14.929249
63.0000	7.0000	75.6 15.049165
64.0000	7.0000	76.8 15.168132
65.0000	7.0000	78.0 15.286174
66.0000	7.0000	79.2 15.403311
67.0000	7.0000	80.4 15.519564
68.0000	8.0000	81.6 15.634953
69.0000	8.0000	82.8 15.749496
70.0000	7.0000	84.0 15.863213
71.0000	7.0000	85.2 15.976119
72.0000	8.0000	86.4 16.088234
73.0000	7.0000	87.6 16.199572
74.0000	7.0000	88.8 16.310151
75.0000	8.0000	90.0 16.419985
76.0000	8.0000	91.2 16.529089
77.0000	8.0000	92.4 16.637478
78.0000	8.0000	93.6 16.745165
79.0000	8.0000	94.8 16.852164
80.0000	8.0000	96.0 16.958487
81.0000	8.0000	97.2 17.064149
82.0000	8.0000	98.4 17.169160
83.0000	8.0000	99.6 17.273533
84.0000	8.0000	100.8 17.377279
85.0000	9.0000	102.0 17.480409
86.0000	8.0000	103.2 17.582934
87.0000	8.0000	104.4 17.684865
88.0000	8.0000	105.6 17.786212
89.0000	9.0000	106.8 17.886984
90.0000	8.0000	108.0 17.987192
91.0000	9.0000	109.2 18.086845
92.0000	8.0000	110.4 18.185952
93.0000	8.0000	111.6 18.284521
94.0000	8.0000	112.8 18.382562
95.0000	9.0000	114.0 18.480083
96.0000	9.0000	115.2 18.577092
97.0000	9.0000	116.4 18.673597
98.0000	9.0000	117.6 18.769606
99.0000	9.0000	118.8 18.865126
100.000 8.0000  120.0 18.960165
